Nested Active-Time Scheduling

The active-time scheduling problem considers the problem of scheduling preemptible jobs with windows (release times and deadlines) on a parallel machine that can schedule up to $g$ jobs during each timestep. The goal in the active-time problem is to minimize the number of active steps, i.e., timesteps in which at least one job is scheduled. In this way, the active time models parallel scheduling when there is a fixed cost for turning the machine on at each discrete step. This paper presents a 9/5-approximation algorithm for a special case of the active-time scheduling problem in which job windows are laminar (nested). This result improves on the previous best 2-approximation for the general case.

==> old-files/LP.tex <==
\subsection{Linear Program}
\label{subsection:linearprogram}

%We begin with a canonical tree.
In the LP, we let $x(i)$ be a variable to represent the time slots opened by node $i$, and let $y(i,j)$ represent the amount of job $j$ that is scheduled in node $i$.  
Recall that the set of tree nodes is $[m]$ and the set of jobs is $J$. The LP is LP \eqref{LP}, which is given in Figure \ref{figure:lp}.



%SHI: it is better to number all the constraints.

\begin{figure}
    \begin{equation}
        \textbf{min} \quad \sum_{i \in [m]} x(i) \quad \textbf{s.t.}  \label{LP}
    \end{equation}\vspace*{-10pt}
    \begin{align}
        \sum_{i \in \Des(K(j)) } y(i, j) &\ge p_j, &\quad &\forall j \label{LPC:scheduled} \\
        \sum_{j \in J(Anc(i))} y(i, j) &\le g \cdot x(i)  &\quad &\forall i \label{LPC:capacity-g} \\
        x(i) &\le L(i)  &\quad &\forall i \label{LPC:capacity-L} \\
        y(i, j) &\le x(i)  &\quad &\forall i, j \label{LPC:y-less-than-x} \\
        y(i, j) &= 0 &\quad &\forall i, j \notin J(Anc(i)) \label{LPC:y-equal-0}  \\
        \sum_{i' \in \Des(i)} x(i') &\ge \ceil{\frac{\sum_{j \in J(\Des(i))} p_j}{g}} &\quad &\forall i \label{LPC:strong}
    \end{align}
    \caption{Linear program for active time scheduling.  %The jobs are numbered $1,2,\ldots,n$ and the nodes in the tree are numbered $1,2,\ldots,m$. The variables are the $x(i)$ and $y(i,j)$.
    By default we restrict $i \in [m]$ and $j \in J$.
    }
    \label{figure:lp}
\end{figure}

The objective is to minimize $\sum_{i \in [m]} x(i)$.
\eqref{LPC:scheduled} ensures that every job $j$ is scheduled in at least $p_j$ time slots.  \eqref{LPC:capacity-g} ensures that the total number of jobs scheduled in $x(i)$ is at most $g \cdot x(i)$, for each node $i \in [m]$. \eqref{LPC:capacity-L} requires that the number of open time slots in a node $x(i)$ is at most the interval length $L(i)$ of node $i$. \eqref{LPC:y-less-than-x} says that we could give at most $x(i)$ time slots for a job $j$. %Otherwise, $y(i,j)$ should be set to $0$. 
\eqref{LPC:y-equal-0} restricts that for each job $j \in J$, $j$ can only be put into nodes in  $\Des(K(j))$.
%
% The second and third constraint says for each node $i$, if we open $x_t$ time slot, it should be less than the interval length $I(i)$ and, the total amount of jobs being put into $x_t$ should be at most $g \cdot x_i$. 
%
\eqref{LPC:strong} is the key that makes the LP stronger: The number of open slots in nodes in $\Des(i)$ should be at least the ceiling of the total volume of jobs belonging to $\Des(i)$ divided by $g$. 

For simplicity, given a node set $V \subset [m]$ and $J' \subset J$, $y(V, J') = \sum_{i \in V, j \in J'} y(i, j)$; If either $V$ or $J'$ is a singleton, we can replace it by the unique element in it.  Recall that $x(S) = \sum_{i \in S} x(i)$ for every $S \subseteq [m]$.

Notice that any solution for the nested active time problem is also a feasible solution for the LP. After running the LP and getting a solution $(x, y)$, we will perform a transformation on the solution.

\begin{lemma} \label{lemma:LPtransform}
Given a feasible LP solution, we can efficiently output another feasible LP solution such that for any pair of nodes $i_1$, $i_2$ such that $i_2 \in \Des^+(i_1)$, if $x(i_2) < L(i_2)$, then $x(i_1) = 0$. 
\end{lemma}
\begin{proof}
    Suppose there are nodes $i_1, i_2$ with $i_2 \in \Des^+(i_1)$ and $x(i_2) < L(i_2)$ and $x(i_1) > 0$.  Then let $\theta = \min\{L(i_2) - x(i_2), x(i_1)\} > 0$. We can move $\theta$ fractional open slots from $i_1$ to $i_2$. For every job $j$, we move $\frac{\theta}{x(i_1)} y(i_1, j)$ fractional assignment of $j$ from $i_1$ to $i_2$. More specifically, let $(x', y') = (x, y)$ initially. We decrease $x'(i_1)$ by $\theta$ and increase $x'(i_2)$ by $\theta$.  For every $j \in J$, we decrease $y'(i_1, j)$ to $\frac{x'(i_1)}{x(i_1)} y(i_1, j)$ and increase $y'(i_2, j)$ to $y'(i_2, j) + \frac{\theta}{x(i_1)}y(i_1, j)$. Notice that every job $j$ that can be assigned to $i_1$ can also be assigned to $i_2$. It is not hard to show that all constraints remain satisfied by the new solution $(x', y')$. Finally we update $(x, y) \gets (x', y')$.
    
    Notice that after the operation, we have either $x(i_1) = 0$ or $x(i_2) = L(i_2)$. By repeating the procedure polynomial number of times, we can find a solution $(x, y)$ satisfying the property of the lemma.
\end{proof}

An example of of the LP transformation is shown in Figure \ref{fig:LPtransformation}.  %The dark slots have at least one job scheduled in them, and the white slots are empty.  After the transformation, in \ref{sublabel2}, the nodes in $R$ are the two nodes in the second level of the tree.
%
%In the Appendix we prove Lemma \ref{lemma:LPtransform} by providing an Algorithm that performs this transformation. % 
Lemma \ref{lemma:LPtransform} implies that for any $i$ with $x(i)>0$, all of its strict Descendants are fully open. We let $I$ be the set of topmost nodes $i$ with $x(i) > 0$. Then the following properties hold:
\begin{itemize}
    \item No node in $I$ is a strict ancestor of another node in $I$.
    \item Any node $i$ with $x(i) > 0$ is a Descendant of some node in $I$. 
    \item For any $i \in I$ and $i' \in \Des^+(i)$, we have $x(i') = L(i')$.
    \item For any $i \in I$ and $i' \in Anc^+(i)$, we have $x(i') = 0$. 
\end{itemize}

%After the LP transformation, we can find a set of nodes $I$ such that all subtrees rooted at $I$ are disjoint and except nodes in $I$, all other nodes in the subtree are full. More precisely, we can always find a set of nodes $I = \{k_1, k_2, ..., k_{|I|}\}$ such that, (1) for each pair $i, i' \in I$, $i \neq i'$, $i \notin \Des(i')$ and $i' \notin \Des(i)$, (2) for all $i \notin \Des(I) $, $x(i) = 0$, and (3) for each $i \in I$ and $i' \in \Des^+(i) $, $x(i') = L(i')$. 

%After identifying the set $I$, we also want to order elements in $I$. We will run depth first search on the tree and the order of $R$ corresponds to the order we traverse the tree. Note that there might be several children for a tree node, we traverse those children based on the increasing order of intervals. Now, given $I = (k_1, k_2, ..., k_{|I|})$, for any $i_1 < i_2 < i_3$, $r_{i_3}$ is not closer to $r_{i_1}$ than $r_{i_2}$ since the lowest common ancestor of $k_{i_1}, k_{i_2}$ is always a \Descendant of that  of $k_{i_1}, k_{i_3}$. 

% For a given node $i$, denote $R(i) = \Des(i) \cap R$ be the nodes in R that are \Descendants of node i. 

We can list all the nodes in $I$ from left to right according to the time horizon. Abusing notations slightly, for any subset $S\subseteq I$, sometimes we also treat $S$ as the sequence of nodes in $S$, using the left-to-right order. Then the distance of two nodes in a sequence $S$ is just the difference between the positions of the two nodes in the sequence.

% Define the time slot for each node $i \in [m]$ as $K(i) = \sum_{j\in \Des(i)} x(j)$. Let $Y(i) = (y(k, j))_{j \in J, k \in \id{\Des(i)}}$ represent the jobs assigned to the time slots in $K(i)$. Given $R$, the set $((i, K(i), Y(i)))_{i \in R}$ defines a LP solution. That's because if $y(k, j)$ is not included in this set, the LP set it to be 0. Given a job $j$, a node $i$, and a job assignment $Y(i)$, the length of the jobs assigned into $i$ is defined as $l(Y(i), j) = \sum_{k \in \id{\Des(i)}} y(k, j)$. For any node $i$, given two job assignments $Y'$ and $Y$, , we say $Y(i) = Y'(i)$, if $l(Y(i), j) = l(Y'(i), j)$ for all $j \in J$.


% Notice that for each $i \in R$, the subtree rooted at $i$ must contain at least one leaf node and all leaf nodes are rigid. Therefore, $K(i) \geq 1$, where $i \in R$. One observation is that all fractional nodes will be only in $R$ because $R$ contains all fractional nodes. If we round up $x_i$ to $\ceil{x_i}$ for all $i \in R$, the total active time slots will be at most $2$ times of the LP solution. This provi\Des us a $2$-approximate algorithm. However, if we want to achieve a better approximation , we have to do more: instead of rounding up all nodes in $R$, we have to round down some $x(i)$ to $\floor{x(i)}$, for $i \in R$. 


% \begin{figure}

%     \subfloat[The open slots from an LP solution]{\label{sublabel1}
%     \includegraphics[width=\linewidth/2]{image1.pdf}}
%     \subfloat[The open slots after performing the LP transformation]{\label{sublabel2}
%     \includegraphics[width=\linewidth/2]{image2.pdf}}
%     \caption{An example of a tree before and after running the LP transformation in Algorithm \ref{alg:transformLP}. The dark slots represent slots have jobs scheduled in them, and the white slots are closed.}
%     \label{fig:LPtransformation}
% \end{figure}


\begin{figure}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{image1.pdf}
        \subcaption{The open slots from an LP solution}\label{sublabel1}
    \end{subfigure}

    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{image2.pdf}
        \subcaption{The open slots after performing the LP transformation}\label{sublabel2}
    \end{subfigure}
    \caption{An example of a tree before and after running the LP transformation in Lemma~\ref{lemma:LPtransform}. %\ref{alg:transformLP}. 
    The dark slots represent slots have jobs scheduled in them, and the white slots are closed.
    }
    \label{fig:LPtransformation}
\end{figure}





==> old-files/algorithm.tex <==
In this section, we describe an algorithm for the trees, as defined in the Section~\ref{section:preliminaries}. The algorithm consists of three phases.
The first phase, described in Section \ref{subsection:linearprogram}, runs a linear program and applies some transformations on the solution.
Section \ref{subsection:rounding} will show the second phase, in which the nodes of the tree are rounded based on the LP solution to find an integral solution.  Finally, to produce the schedule of the jobs, a max-flow computation can be run on the set of jobs and set of open time slots found in phase 2.  See the Appendix A.1 of \cite{Kumar18} for the specification of the max-flow computation to produce the schedule of jobs.



==> old-files/analysis.tex <==

\label{section:analysis}
Next, we will show that the rounding time slot $\tilde x$ is a feasible solution. 
\subsection{Feasibility of $\tilde x$}
First we will give an if-and-only-if condition
\begin{lemma}
\label{ifandonlyif}
    Given an integer solution $\tilde x$ for the LP, $\tilde x$ is feasible if and only for every subset $J' \subseteq J$ of jobs, we have 
	\begin{align*}
		\sum_{i \in [m]} \min\{|J'(\Anc(i))|, g\} \cdot \tilde x(i) \geq p(J'),
	\end{align*}
% 	where $J'_i = J' \cap J_i$ for every $i \in [m]$ and $J'(S)$ for any $S \subseteq [m]$ is defined as $\union_{i \in S}J'_i = J(S) \cap J'$ using the shorthand rule.
\end{lemma}
\begin{proof}
Recall $J'(\Anc(i)) = \union_{i' \in \Anc(i)} J'(i')$ is the set of jobs in $J'$ that can be assigned to $i$. The only if part is easy to see. Any node $i$ can hold at most $\min\{|J'(\Anc(i))|, g\} \cdot \tilde x(i)$ volume of jobs in $J'$. All the jobs in $J'$ should be assigned. If $\tilde x$ is feasible, then $\sum_{i \in [m]} \min\{|J'(\Anc(i))|, g\} \cdot \tilde x(i) \geq p(J')$.

Now we prove the if part, by considering the contra-positive of the statement and applying the maximum-flow-minimum cut theorem. Assume $\tilde x$ is not feasible. 
We construct a 4-layer directed network $H = (V_H, E_H)$, where the nodes from left to right are $\{s\}, J, [m] $ and $\{t\}$. There is an edge from $s$ to every $j \in J$ with capacity $p_j$, an edge from every $j \in J$ to every $i \in \Des(k(j))$ with capacity $\tilde x(i)$, and an edge from every $i \in [m]$ to $t$ with capacity $g\cdot \tilde x(i)$. For a subsets $V'\subseteq V_H$ and a node $v \in V_H \setminus V'$, we use $E_H(V', v)$ to denote the set of edges from $V'$ to $v$. 

As $\tilde x$ is not feasible, there is a $s$-$t$ cut in the network has capacity less than $p(J)$. Let $(A, B)$ be the cut: $s \in A, t \in B$ and $A \uplus B = V_H$ . Its cut value, which is
$p(B \cap J) + \sum_{i \in B \cap [m]}|E_H(A \cap J, i)|\cdot \tilde x(i) + g\cdot \tilde x(A \cap [m])$, is less than $p(J)$. This is equivalent to 
$\sum_{i \in B \cap [m]} |E_H(A \cap J, i)|\cdot \tilde x(i) + g\cdot \tilde x(A \cap [m]) < p(A \cap J)$. Let $J' = A \cap J$. Then the contribution of a node $i \in [m]$ to the left-side is either $|E_H(J', i)|\cdot\tilde x(i)$ (if $i \in B$), or $g \cdot \tilde x(i)$ (if $i \in A$), which is lower bounded by $\min\{|E_H(J', i)|, g\}\cdot \tilde x(i)$. Noticing $|E_H(J', i)| = |J'(\Anc(i))|$, we have $\sum_{i \in [m]} \min\{|J'(\Anc(i))|, g\}\cdot \tilde x(i) < p(J')$. This finishes the proof of the if part. 
%
%Proof by contradiction. Assume that the minimum cut is smaller than $p(J)$, then it must contains only part of edges between first to the second layer. Consider job set $\Bar{J}$ where there is no cut from $s$ to jobs in and consider node $i$ in the third layer. If we want to cut the link from $s$ to $i$ to $t$, we could either remove all incoming edges from $J'$ or outgoing edges to $t$. Notice that we add at least $\min\{|\Bar{J}(\Anc(i))|, g\} \cdot \tilde x(i)$ to the cut. In total, the value of this cut is at least $p(J \setminus \Bar{J}) + \sum_{i \in \Bar{J}} \min\{|\Bar{J}(\Anc(i))|, g\} \cdot \tilde x(i) \geq p(J)$, contradicts to the fact of minimum cut. Therefore, if the inequality holds, then, $\tilde x$ is feasible. 
\end{proof}
Once we have the if-and-only-if condition for the feasibility, the main lemma we need to prove is the following:
	\begin{theorem}
		\label{thm:covering}
		For every subset $J' \subseteq J$ of jobs, we have 
	\begin{align}
		\sum_{i \in [m]} \min\{|J'(\Anc(i))|, g\} \cdot \tilde x(i) \geq p(J'), \label{inequ:covering}
	\end{align}
	\end{theorem}
	
% 	Using the maximum flow minimum cut theorem, we can show that $\tilde x$ is valid if and only if the condition in Theorem~\ref{thm:covering} holds.  Therefore it remains to prove the theorem.
	
	 The rest of the section is dedicated to the proof of Theorem~\ref{thm:covering}. From now on we fix a subset $J' \subseteq J$ and prove \eqref{inequ:covering}. For notational convenience, let  $u_i = \min\{|J'(\Anc(i))|, g\}$ and $w_i = u_i x(i)$ and $\tilde w_i = u_i \tilde x(i)$ for every $i \in [m]$. Thus, \eqref{inequ:covering} is simply written as $p(J') \leq \tilde w([m])$. Recall that $y(V, J') = \sum_{i \in V, j \in J'} y(i, j)$ for a given $V \subseteq [m], J' \subseteq J$. We have $p(J') = y([m], J') = y(\Des(I), J')$ and $\tilde w([m]) = \tilde w(\Des(I))$. Thus, we need to prove $y(\Des(I), J') \leq \tilde w(\Des(I))$.

	\begin{claim}
		\label{claim:simple}
		For every $i \in [m]$, we have $y(i, J') \leq w_i = u_i x(i)$. 
	\end{claim}
	\begin{proof}
		If $u_i = g$, we use the \eqref{LPC:capacity-g} in the LP. If $u_i < g$, then we use \eqref{LPC:y-less-than-x} and \eqref{LPC:y-equal-0}.
	\end{proof}

Below, for a subset $S$ of $I$, and a list $\Pi$ of types, let $S_\Pi$ be the set of nodes in $S$ that is of type $\pi$ for some $\pi \in \Pi$.  For example, $S_{\sfA, \sfC_1}$ is the set of nodes in $S$ of type $\sfA$ or $\sfC_1$. We shall define more types for nodes in $I$ and this definition extends to the new types.

	We handle nodes in $\Des(I_\sfB)$ directly:
	\begin{coro}
		$y\big(\Des(I_\sfB), J'\big) \leq \tilde w\big(\Des(I_\sfB)\big) $.
	\end{coro}
	\begin{proof}
		This is by Claim~\ref{claim:simple} and that for every $i \in \Des(I_\sfB)$, we have $x(i) \leq \tilde x(i)$. 
	\end{proof}
	
	Thus, to prove \eqref{inequ:covering} it remains to prove 
	\begin{align}
		y\big(\Des(I_{\sfA, \sfC}), J'\big) \leq \tilde w\big(\Des(I_{\sfA, \sfC})\big). 
		\label{inequ:remaining}
	\end{align}
	
	%TODO: Only consider A, C types.
	
	For any node $i \in I$, we say $i$ is of type-$\sfg$ if $u_i = g$ and $i$ is of type-$\sfs$ if $u_i < g$.  (Think of ``$\sfg$'' as the parameter $g$, and ``$\sfs$'' as ``smaller-than $g$''.) Unlike type-$\sfA$, $\sfB$ and $\sfC_1$ and $\sfC_2$ nodes, the definitions of type-$\sfg$ and $\sfs$ nodes depend on the chosen set $J'$ in our analysis.
	
	Based on the two definitions of types, we define conjunctive types. For example, a type-$\sfC_2\sfg$ node is a node in $I$ that is of type-$\sfC_2$ and type-$\sfg$.  \medskip
	
    Let $I' \subseteq I$; recall that $I'$ can be viewed as a sequence. We define a segment $S$ in $I'$ as a sub-string of the sequence $I'$. Again, we view $S$ both as a sequence and as a set.
	\begin{lemma}
		\label{lemma:mark}
		Let $S$ be a segment in $I_{\sfA,\sfC}$ with $|S_{\sfA\sfg, \sfC_2\sfg}| \geq 1$ and $|S_{\sfA\sfg, \sfC_2\sfg}| + 1 \geq |S_{\sfC_1}|$. Then,  we have 
		\begin{align*}
			y\big(\Des(S)), J'\big) \leq  \tilde w\big(\Des(S))\big).
		\end{align*}
	\end{lemma}
	\begin{proof}
	    By Claim~\ref{claim:simple}, we have $y\big(\Des^+(S)), J'\big) \leq w(\Des^+(S)) = \tilde w(\Des^+(S))$. So it remains to prove $y(S, J') \leq \tilde w(S)$. As $y(S, J') \leq w(S)$, it suffices to prove $w(S) \leq \tilde w(S)$. Recall that $S \subseteq I_{\sfA, \sfC}$.
		\begin{itemize}
			\item If $i \in S_{\sfC_1}$, $w_i - \tilde w_i \leq 0.2 u_i \leq 0.2g$.
			\item If $i \in S_{\sfC_2\sfs, \sfA\sfs}$, then we have $w_i \leq \tilde w_i$.
			\item If $i \in S_{\sfC_2\sfg,\sfA\sfg}$, we have $\tilde w_i  - w_i \geq 0.4g$.
		\end{itemize}
		Therefore, a type-$\sfA\sfg$ or $\sfC_2\sfg$ node can cover two type-$\sfC_1$ nodes. The lemma follows as its conditions imply that $|S_{\sfC_1}| \leq 2|S_{\sfA\sfg, \sfC_2\sfg}|$.
	\end{proof} 
	
		
	We \emph{mark} some disjoint segments $S$ in $I_{\sfA, \sfC}$ satisfying the property of Lemma~\ref{lemma:mark} as follows.  We partition the sequence $I_{\sfA, \sfC}$ into sub-strings by removing nodes in $I_{\sfC_1}$. If an interval contains at least one node of type $\sfC_2\sfg$ or $\sfA\sfg$, the whole sub-string along with possibly the two type-$\sfC_1$ nodes to its left and right will be marked. All the other nodes in $I_{\sfA, \sfC}$ are unmarked. Clearly marked nodes in the sequence $I_{\sfA, \sfC}$ form many separated segments in $I_{\sfA, \sfC}$, each of which satisfy the conditions of Lemma~\ref{lemma:mark}. A maximal unmarked segment only contains nodes in $I_{\sfA_\sfs, \sfC_2\sfs, \sfC_1}$. Let $I^\marked$ and $I^\unmarked$ be the set of marked and unmarked nodes in $I_{\sfA, \sfC}$. See Figure~\ref{fig:segments} for an example of how we mark nodes.
	\begin{figure*}
	    \includegraphics[width=0.75\textwidth]{segments}
	    \caption{Illustration of $I^\marked$ and $I^\unmarked$.} \label{fig:segments}
	\end{figure*}
	
	We say a job $j$ is local if $k(j) \in \Des(i)$ for some type-$\sfC_1$ node $i$. In this case $j$ we must have $p_j = 1$, since otherwise we would have $\tilde x(\Des(i)) \geq 2$, contradicting that $i$ is of type $\sfC$.  Let $J'_{\local}$ be the set of local jobs in $J'$.
	
	\begin{lemma}
		\label{lemma:unmark}
		Let $j \in J' \setminus J'_\local$. Let $S$ be a maximal segment in $I_{\sfA, \sfC}$ that contains only nodes in $I^\unmarked \cap \Des(k(j))$. (This implies that $S_{\sfA, \sfC_2} = S_{\sfA\sfs, \sfC_2\sfs}$.) Then we have 
		\begin{align}
			y\Big(\Des(S), j\Big)  \leq \tilde x\big(\Des(S_{\sfA, \sfC_2})\big). \label{inequ:y-to-tildex-non-local}
		\end{align}
	\end{lemma}
	\begin{proof} 
		By \eqref{LPC:y-less-than-x} in the LP, we have $y\Big(\Des(S), j\Big)  \leq x\big(\Des(S)\big)$. If we can prove 
		\begin{align}
			x\big(\Des(S)\big) \leq \tilde x\big(\Des(S_{\sfA, \sfC_2})\big), \label{inequ:x-to-tildex-non-local}
		\end{align}
		then we proved the lemma. 

		Notice that
		\begin{enumerate}[label=(P\arabic*)]
			\item A type-$\sfC_1$ node $i \in S$ has $x(\Des(i)) < 1.2$.
			\item A type-$\sfC_2$ node $i \in S$ has $\tilde x(\Des(i)) - x(\Des(i)) \geq 0.8$.
			\item A type-$\sfA$ node $i \in S$ has $\tilde x(\Des(i)) - x(\Des(i)) \geq 0.4$.
		\end{enumerate}
		Moreover, in the sequence $S$, between any two type-$C_1$ nodes, there are at least two type-$C_2$ nodes.  Also, $j$ is not local and thus it can be assigned to at least two nodes in $I$. For easy of notation, let $n_{\sfC_1} = |S_{\sfC_1}|$, $n_{\sfC_2} = |S_{\sfC_2}|$, $n_{\sfA} = |S_{\sfA}|$. 
		
		First consider the case where $S$ is also a segment in the whole sequence $I$, and both the node $v$ to the left of $S$ in $I$ and the node $v'$ to the right of $S$ are not type-$\sfB$ nodes that $j$ can be assigned to. Then the node $v$ ($v'$ resp.) is either nonexistent, or of type-$\sfC_1$, or a node that $j$ can not be assigned to: Assuming otherwise, $v$ ($v'$) is a type-$\sfA, \sfB$ or $\sfC_2$ node that $j$ can be assigned to. By our assumption it can not be of type-$\sfB$ and so it must be a type-$\sfA$ or $\sfC_2$ node that $j$ can be assigned to. But in this case $v$ ($v'$) should have been included in $S$. 
		
		
		We consider many cases:
		\begin{itemize}
		    \item Both $v$ and $v'$ are nodes that $j$ can not be assigned to (if a node does not exist, the condition also holds). In this case, $\Des(S)$ is everything that $j$ can be assigned to.  
		    Then we have $y(\Des(S), j) = p_j \leq \floor{1.2 n_{\sfC_1} + x(\Des(S_{\sfA, \sfC_2}))}$, and $\tilde x(\Des(S_{\sfA,\sfC_2})) = \floor{x(\Des(S_{\sfA,\sfC_2}))} + n_{\sfA} + n_{\sfC_2}$.
		
		    
		    
		    \begin{itemize}
		        \item $n_{\sfC_1} = 1$, $n_{\sfC_2} = 0$, $n_{\sfA} = 1$. \eqref{inequ:y-to-tildex-non-local} holds as $\floor{1.2 + 0.6} = 1$.
		        \item $n_{\sfC_1} = 1$, $n_{\sfC_2} = 0$, $n_{\sfA} = 2$. \eqref{inequ:y-to-tildex-non-local} holds as $\floor{1.2 + 0.6\times 2} = 2$.
		        \item $n_{\sfC_1} = 1$, $n_{\sfC_2} = 1$, $n_{\sfA} = 0$. \eqref{inequ:y-to-tildex-non-local} holds as $\floor{1.2 + 0.2} = 1$.
            \item In all other cases with $n_{\sfC_1} = 1$, we have $0.4n_{\sfA} + 0.8n_{\sfC_2} \geq 1.2 n_{\sfC_1}$. Then \eqref{inequ:x-to-tildex-non-local} holds by (P1), (P2) and (P3). 
            \item $n_{\sfC_1} = 2$, $n_{\sfC_2} = 2$, $n_{\sfA} = 0$. \eqref{inequ:y-to-tildex-non-local} holds 
            as $\floor{2.4 + 0.2 \times 2} = 2$.
            \item $n_{\sfC_1} = 2$, $n_{\sfC_2} = 2$, $n_{\sfA} = 1$. \eqref{inequ:y-to-tildex-non-local} holds 
            as $\floor{2.4 + 0.2 \times 2 + 0.6} = 3$.
            \item Notice that we when $n_{C_1} = 2$ we have $n_{C_2} \geq 2$. So, in all other cases with $n_{C_1}=2$, we have $0.4n_{\sfA} + 0.8n_{\sfC_2} \geq 1.2 n_{\sfC_1}$. Again \eqref{inequ:x-to-tildex-non-local} holds.
            \item $n_{\sfC_1} = 3$, $n_{\sfC_2} = 4$, $n_{\sfA} = 0$. \eqref{inequ:y-to-tildex-non-local} holds as
            $\floor{3.6 + 0.2\times 4} = 4$.
            \item In all other cases with $n_{\sfC_1} = 3$, we have $0.4n_{\sfA} + 0.8n_{\sfC_2} \geq 1.2 n_{\sfC_1}$ and thus \eqref{inequ:x-to-tildex-non-local} holds.
            \item $n_{\sfC_1} \geq 4$. Then $n_{\sfC_2} \geq 2(n_{\sfC_1} - 1) \geq \frac32 n_{\sfC_1}$. $0.4n_{\sfA} + 0.8n_{\sfC_2} \geq 1.2 n_{\sfC_1}$ and thus \eqref{inequ:x-to-tildex-non-local} holds.
		    \end{itemize}
		    \item At least one of $v$ and $v'$ is a type-$\sfC_1$ node.  Then we have $n_{\sfC_2} \geq 2n_{\sfC_1}$ and \eqref{inequ:x-to-tildex-non-local} holds.
		\end{itemize}
		
    %   \begin{itemize}
    %      \item $n_{\sfC_1} = 1$. In this case,  since otherwise $j$ would be a local job. 

    %   \end{itemize}
      
      Now consider the remaining case that either $S$ is not a segment in the sequence $I$, or $v$ or $v'$ is a type-$\sfB$ node that $j$ can be assigned to. In the former case, let $v^*$ be any node that breaks $S$ in $I$. Notice that $v^*$ is a type-$\sfB$ node that $j$ can be assigned to. In the latter case, let $v^*$ be $v$ or $v'$, whichever is the type-$\sfB$ node that $j$ can be assigned to.  Node $v^*$ forced two type-$\sfC$ nodes to be rounded up. By the way we choose the two nodes, the following is true: either there are no type-$\sfC_1$ nodes in $S$, or both forced nodes are in $S$. In the former case, \eqref{inequ:x-to-tildex-non-local} clearly holds. In the latter case, we have $n_{\sfC_2} \geq 2(n_{\sfC_1} + 1) + 2 = 2n_{\sfC_1}$. Then \eqref{inequ:x-to-tildex-non-local} holds due to (P1), (P2) and (P3). 
%       In both cases, either all type-$\sfC$ nodes in $S$ are type-$\sfC_2$ or at least two type-$\sfC_2$ nodes is affected by a type-$\sfB$ nodes. If $S$ is not an interval in the sequence $I$, let $i$ be the node in the sequence $I$ but not covered by $S$, then $i$ is not a type-$\sfA$ or type-$\sfC$ nodes, otherwise $i$ will be included in $S$. $i$ will force two closest nodes(or $S$ contains only one type-$\sfC$ node) to be type-$\sfC_2$ and both nodes will be included in $S$. In the other case, if $v$ or $v'$ is a type-$\sfB$ node, again $v$ or $v'$ will force two closest nodes to be type-$\sfC_2$ nodes, since job $j$ can be assigned to $v$ or $v'$, then both nodes will be included in $S$. In either case, at least two type-$\sfC_2$ nodes in $S$ are affected by a type-$\sfB$ node or $S$ contains only one type-$\sfC$ node and that node is type-$\sfC_2$. If $S$ contains only one type-$\sfC$ node, since this node is type-$\sfC_2$, then the inequality holds automatically.
%
% 	   For the first situation, consider type-$\sfC$ nodes which is not affected by type-$\sfB$ nodes, let $(l_1, l_2, ..., l_{\rho})$ be those nodes in $S$ from left to right. Note that all type-$\sfC_1$ nodes are in this sequence and between any two adjacent $\sfC_1$ nodes, there are at least two $\sfC_2$ nodes. Combining those points together, $\sum_{l_i \in S_{\sfC_2}}{\tilde x(l_i)} - \sum_i(x(l_i)) \geq -1.2$. Notice we have at least two nodes affected by type-$\sfB$ node in $S$ and each can contribute $0.8$. $x\big(S_{\sfA, \sfC_2}\big) - x\big(\Des(S)\big) \geq -1.2 + 0.8 \times 2 \geq 0$ holds.
%  %       
  %      Notice that job j can be fitted into a segment of $I$. If $y\Big(\Des(S), j\Big)$ is not integer, then part of job $j$ is assigned to some node $i'$ outside of $S$. Assume that $i'$ is on the left of $S$ in $I$.
   %     \begin{itemize}
%            \item If $i'$ is type-$\sfA\sfg$ or type-$\sfC_2\sfg$, then $i'$ rules out the first type-$\sfC_2$ node in $S$
%            \item If $i'$ is type-$\sfA$ or type-$\sfC_2$, then $i'$ is included to $S$, contradicting to the fact $i'$ is outside of $S$.
        %     \item If $i'$ is type-$B$, then $B$ will force two type-$\sfC$ nodes to be type-$\sfC_2$ and both will be included in the $S$ on the left side.
        %     \item If $i'$ is type-$\sfC_1$ node, then there will be at least 2 type-$\sfC_2$ nodes between $i'$ and the first type-$\sfC_1$ node, i.e, $l_1, l_2$.  
        % \end{itemize}
        %   In either case, we have $l_1, l_2$ or $l_{\rho - 1}, l_{\rho}$ is type-$\sfC_2$ nodes. These two nodes will contributes $0.8 * 2 = 1.6$ and other part consume at most $-1.2$ for $\tilde x(i) - x(i)$. Therefore, if $y\Big(\Des(S), j\Big)$ is not integer, we always have $x\big(\Des(S)\big) \leq \tilde x\big(S_{\sfA, \sfC_2}\big)$.
  %        
        %   The final case is that $y\Big(\Des(S), j\Big)$ is an integer. Note that $S$ contains at least one type-$\sfC_2$ node, otherwise, $j$ will be a local job. , recall each adjacent type-$\sfC_1$ nodes contains 2 type- each $\sfC_2$ nodes and, type-$\sfC_1$ requests 1.2 and each type-$\sfC_2$ contributes 0.8 and each type-$\sfA$ provides 0.4. There are several cases
        %   Combining all cases, we have $y\Big(\Des(S), j\Big)  \leq \tilde x\big(S_{\sfA, \sfC_2}\big)$.
%
%		
%		
% 		By some tedious case-by-case analysis, if the inequality does not hold. The sequence $S_{\sfC_1, \sfC_2}$ must  be one of the following two cases:
% 		\begin{enumerate}
% 			\item $\sfC_1, \sfC_2$. (The other case $\sfC_2, \sfC_1$ is symmetric.)
% 			\begin{itemize}
% 				\item If some type-$\sfB$ node is involved, then this can not happen since the type-$\sfB$ node will force two type-$\sfC$ nodes to be rounded up. 
%				
% 				\item If $S$ does not contain other node, then $p_j = 2$ the lemma is proved. 
%							
% 				\item If $S$ contains a node of type $\sfA$ $i$, then the inequality can be proved as if  an integer is less than $0.6 + 1.2 + 1.2$, then it is at most $3$. 
% 			\end{itemize}			
% 			\item $\sfC_1, \sfC_2, \sfC_2, \sfC_1$
% 			\begin{itemize}
% 				\item Again, if there is a type-$\sfB$ node involved, then the case can not happen. 
% 				\item If $S$ does not contain other nodes, then $p_j < 4\times 1.2 = 4.8$ and thus $p_j \leq 4$.  The inequality holds.
% 				\item $S$ contains one type-$\sfA$ node. $\floor{4.2 + 0.6} = 4 \leq 5$. 
% 				\item $\cdots$.
% 			\end{itemize}
%			
% 		\end{enumerate}
\end{proof}
	
\textbf{Proof of Inequality~\eqref{inequ:remaining}}
	
Summing up the inequality of Lemma~\ref{lemma:mark} over all maximal marked segments $S$ in $I_{\sfA, \sfC}$, we have 
	\begin{align*}
		y\big(\Des(I^\marked), J'\big) \leq \tilde w\big(\Des(I^\marked)\big).
	\end{align*}
	
	
	Summing up the inequality of Lemma~\ref{lemma:unmark} over all jobs $j \in J' \setminus J'_\local$ and relevant $S$, we have
	\begin{align*}
		y(I^\unmarked \cup \Des^+(I^\unmarked_{\sfC_1}), J' \setminus J'_{\local}) \leq \tilde w\big(I^\unmarked_{\sfA, \sfC_2}\big).
	\end{align*}
	This holds since for every $i \in S_{\sfA, \sfC_2}$, $\tilde x_i$ only appears $u_i < g$ times on the right side of the inequality in Lemma~\ref{lemma:unmark}. 
			
	Finally, we have 
	\begin{align*}
		y(I^\unmarked \cup \Des^+(I^\unmarked_{\sfC_1}), J'_{\local}) \leq \tilde w(\Des(I^\unmarked_{\sfC_1})),
	\end{align*}
	because of the last inequality of the LP. 
	
	Overall, adding all the inequalities together, we have $y(I_{\sfA,\sfC} \cup \Des^+(I_{\sfC_1}), J') \leq \tilde w(I_{\sfA,\sfC} \cup \Des^+(I_{\sfC_1}))$, which is precisely \eqref{inequ:remaining}.
	
	Combining all components together, we have the following theorem for the feasibility.
	\begin{theorem}
	The vector $\tilde x$ produced by the rounding algorithm is a feasible solution for the scheduling instance.
	\end{theorem}
	
% In this section, we will show the following theorem. 
% \begin{theorem}
% \label{1.75main}
% There exists 5/3-approximation polynomial-time algorithm for the nested active-time problem.
% \end{theorem}

% First we will show that after running the algorithm, the number of open time slots in the solution is at $\alpha$ times the LP solution, for any $\alpha \geq 1.5$.

% \begin{lemma}
% For any $\alpha \geq 1.5$, after running the Algorithm \ref{alg:rounding}, $\sum_{i} t'(i) \leq \alpha \sum_{i} k(i)$.
% \end{lemma}
% \begin{proof}
% When we process the nodes from $R$, rounding up nodes with $k(i) \in \{1 \} \cup [2, +\infty)$ never violates the ratio whenever $\alpha \geq 1.5$. Next, for each internal node, we will only round up a node if rounding one node doesn't violate the ratio, so our ratio is at most $\alpha$.
% \end{proof}

% Next we want to argue that we produce a feasible solution.  We will only show that the algorithm produces a feasible solution for $\alpha \geq 1.75$.
% To show that the set of time slots produced by the algorithm is a feasible solution, we will give an assignment of jobs $Y'(i)$ for each node and its open time slots $(i, t'(i))$. 
% For each node $i$, we will set up a potential value $\Delta(i)$ to record the unused space of the time slot in $R(i)$.  Intuitively, when $\Delta(i) < 0$, we need an extra $\Delta(i)$ space to hold the jobs assigned to $Y(k)$, where $k \in R(i)$, and when $\Delta(i) > 0$, there is $\Delta(i)$ open time slots to fit other jobs in. 
% More precisely, for any node $i \in R$ such that $\id{state}(i) = \id{up}$, set $\Delta(i) = t'(i) - k(i)$.
% Notice that if a node $i$ is rounded up, the jobs can be scheduled in the node as they were according to transformed LP solution.  Set $Y'(i) = Y(i)$ and there is $\Delta(i)$ unused open time slots left. 
% For the case where a node $i \in R$ has $\id{state}(i) = \id{down}$, set $\Delta(i) = -k(i)$. For an internal node $i$, set $\Delta(i) = \Delta(i.\id{left}) + \Delta(i.\id{right}) = \sum_{j \in R(i)} \Delta(j)$.


% For a node $i$ with $\Delta(i) < 0$, we need some extra space to fit all jobs in the $R(i)$.  Recall that $Y(i)$ is the assignment of jobs to the time slots in node $i$ after running the LP and the LP transform.
% Fortunately, we don't need to schedule all jobs from $(Y(k))_{k \in R(i)}$ in the new time slot of $R(i)$. Instead we will schedule all the jobs in 
% $J(\id{Des}(i))$, and only part of the jobs in $J(\id{Anc}(i) \backslash \{i\})$.  We allow up to $\Delta(i)$ time slots of the jobs in $J(\id{Anc}(i) \backslash \{i\})$ to be scheduled later.  Since these jobs come from ancestor nodes, they are allowed to be scheduled above $i$, once there is extra space for them to fit.

% \begin{definition}
% For a node $i$ with $\Delta(i) < 0$, we say $i$ is  $\Delta$-scheduled if there is a job assignment $Y'(i)$ such that the following hold.
% \begin{itemize}
%     \item For jobs $j$ from $J(\id{Des}(i))$, it must have been scheduled entirely in the time slot $k \in R(i)$ in the LP solution, so we require it is scheduled entirely in $Y'(i)$, i.e, $l(Y'(i), j) = l(Y(i), j$ for all $j \in J(\id{Des}(i))$.
%     \item For job $j$ from $J(\id{Anc}(i) \backslash \{ i \})$, part of or the entire job is scheduled in $Y(i)$ for the original LP, so we require that $Y'(i)$, $l(Y(i), j) - l(Y'(i), j) \leq |\Delta(i)|$ and $\sum_{j \in J(\id{Anc}(i) \backslash \{ i \})}(l(Y(i), j) - l(Y'(i), j)) \leq g \cdot |\delta(i)|$. In other words, 
%     for the jobs from $J(\id{Anc}(i) \backslash \{ i \})$  assigned to a time slot in $R(i)$, we only need an extra time slot with length $|\Delta(i)|$ to hold it.
% \end{itemize}
% \end{definition}
% Note that, for the job $j \in J(\id{Anc}(i) \backslash \{ i \})$, we don't require the whole job is scheduled into $Y'(i)$, we only require at least $l(Y(i), j) - |\Delta(i)|$ length can fit in $Y'(i)$.



% Now consider the set of nodes $i$ with $\Delta(i) < 0$, which are highest in the tree, i.e. denote $D = \{i_1, i_2, ..., i_k \} \subset [m]$ such that, (1) for any $i \in D$, $\Delta(i) < 0$, (2) for any $d_i, d_j \in D$, $i \neq j$, $d_i \notin \id{Des}(d_j)$ and $d_j \notin \id{Des}(d_i)$,  and (3) for all $i \in [m] \backslash \id{Des}(D)$, $\Delta(i) \geq 0$.
% % \begin{itemize}
% %     \item for any $i \in D$, $\Delta(i) < 0$,
% %     \item for any $d_i, d_j \in D$, $i \neq j$, $d_i \notin \id{Des}(d_j)$ and $d_j \notin \id{Des}(d_i)$ and,
% %     \item for all $i \in [m] \backslash \id{Des}(D)$, $\Delta(i) \geq 0$.
% % \end{itemize}
% $D$ is the set of nodes $i$ such that each $\Delta(i)$ is negative and they are the highest possible nodes in the tree. For any given node $i$, if $\Delta(i) < 0$ and $\Delta(k) \geq 0$ for all $k \in \id{Anc}(i) \backslash \{ i \}$, then $i \in D$.

% We want to show that for nodes $i$ with $\Delta(i) \geq 0$,  we can schedule the jobs that were initially put in the node by the LP after the transformation.  
% In the following lemma, we show how to move jobs between nodes that are $\Delta$-scheduled, and have open time slots.


% Once we define scheduled node with negative $\Delta$ value and $D$ set, we have the following Lemma.
% \begin{lemma}
% \label{allnodesscheduled}
% If for all $d \in D$, $d$ is $\Delta$-scheduled, then for any node $i \in [m]$ such that $\Delta(i) \geq 0$ and $i \notin \id{Des(D)}$, there is a job assignment $Y'$ such that $Y'(i)  = Y(i)$ and $Y'(i)$ can provide unused time slot with length $\Delta(i)$.
% \end{lemma}

% \begin{proof}
% Proof by induction. The base case is the node $i$ from $R$ such that $i \notin \id{Des}(D)$. Since $\Delta(i) \geq 0$, the state of $i$ is rounded up. We will set $Y'(i)$ as $Y(i)$ for time slot $k(i)$ and we still have $x'(i) - x(i) = \Delta(i)$ unused time slot.


% Now, for any node $i$ such that $\Delta(i) \geq 0$ and $i \notin \id{Des}(D)$. Assuming that we already prove the lemma holds for $\id{Des}(i) \backslash \{ i \}$. If $i$ only contains one child node, we already set up the assignment and $i$ still has $\Delta(i.\id{child}) = \Delta(i)$ unused time slot. Otherwise, $i$ has two children. 
% If both children's $\Delta$ value is greater or equal to 0. We again don't do any thing and the assignment for the children can provide $\Delta(i.\id{left}) + \Delta(i.\id{right}) = \Delta(i)$ unused time slot. Otherwise, one of the children's $\Delta < 0$, assume $\Delta(i.\id{left}) < 0$. 
% Because the $\Delta$ value of $\id{Anc}(i) \backslash \{ i \}$ is non-negative, we know $i.\id{left}$ must be in $D$. 
% We already know there is job assignment $Y'(i.\id{left})$ for $i.\id{left}$ such that we only needs an extra $|\Delta(i.\id{left})|$ to hold jobs from $J(\id{Anc}(i.\id{left} \ \{ i.\id{left} \}) = J(\id{Anc}(i))$. 
% We could move those jobs into the right child time slot because all the jobs need to be assigned are from $\id{Anc}(i)$. The last point is that we already know $\Delta(i) = \Delta(i.\id{left}) + \Delta(i.\id{right}) \geq 0$, the right child time slot is enough to hold unassigned jobs from left side and after assignment, we still have $\Delta(i.\id{right}) - |\Delta(i.\id{left})| = \Delta(i)$ unused time slot. 
% \end{proof}



% For nodes $i$ where $|R(i)|$ is large enough, the problem is slightly easier.  In the next lemma, we show that any nodes where $|R(i)|$ is of sufficient size have $\Delta(i) \geq 0$.  
% The analysis for small $|R(x)|$ gets more difficult and much more complicated.  We have to show that $x$ is $\Delta$-scheduled.



% Now we already show if $D$ can be scheduled, all nodes can be scheduled, too. Hence, our following lemma will identify $D$.


% \begin{lemma} \label{lemma:positivedelta}
% if $\alpha \in (5/3, 2)$, for each node $i$ such that $(2\alpha - 1)\floor{\alpha |R(i)|} -2\alpha|R(i)| \geq 1$, $\Delta(i) \geq 0$.
% \end{lemma}

% The proof of Lemma \ref{lemma:positivedelta} is deferred to the Appendix.  
% The proof shows that for any $i$ such that $\Delta(i) < 0$, $\Delta(i)$ is minimized if $j \in R(i)$, $k(j) \in (1, 2)$.  Then, the algorithm can only round up as many nodes as possible in $R(i)$ until violating the approximation ratio $\alpha$, and the rest of the nodes in $R(i)$ are rounded down.  
% Since each node $x$ in $R(i)$ has $k(j) \in (1, 2)$,  this gives a bound within one of the number of nodes rounded down in $R(i)$.  With this limit on the number of nodes rounded down, there are enough nodes in $R(i)$ that are rounded up so that $\Delta(i) \geq 0$.
% % To show that $\Delta(i)$ is minimized when all $x \in R(i)$, $k(x) \in (1, 2)$, we compare a set of nodes which are identical except for 



% We can have the simpler constraint for $|R(i)|$ by using $\floor{\alpha |R(i)|} \geq \alpha |R(i)| - 1$. 
% \begin{equation*}
% \begin{aligned}
%     (2\alpha - 1)\floor{\alpha |R(i)|} -2\alpha|R(i)| - 1 &\geq (2\alpha - 1)(\alpha |R(i)| - 1) -2\alpha|R(i)| - 1 \geq 0 \\
%     \Rightarrow |R(i)| &\geq \frac{2}{2\alpha - 3}
% \end{aligned}
% \end{equation*}
% Thus, if $|R(i)| \geq \frac{2}{2\alpha - 3}$, $\Delta(i) \geq 0$. For $\alpha \geq 1.75$, we get $|R(i)| \geq 2 / (2 \cdot 1.75 -3) = 4$. Notice that if $|R(i)| = 3$, we still have $(2\alpha - 1)\floor{\alpha|R(i)|} - 2\alpha|R(i)| \geq 1$ for all $\alpha \geq 7/4$, we get the following corollary,
% \begin{corollary}
% \label{175rsize}
% If $\alpha \in [7/4, 2)$, after we finish the algorithm, for any give node $i$ such that $|R(i)| \geq 3$, we have $\Delta(i) \geq 0$.
% \end{corollary}
% % \begin{corollary}
% % \label{53rsize}
% % If $\alpha \in [5/3, 7/4)$, after we finish the algorithm, for any give node $i$ such that $|R(i)| \geq 5$, we have $\Delta(i) \geq 0$.
% % \end{corollary}
% % For $\alpha \in [5/3, 7/4)$, when $|R(i)| = 3$, $(2\alpha - 1)\floor{\alpha |R(i)|} -2\alpha|R(i)| \geq 1$ is satisfied. Thus, we only have negative $\Delta(i)$ for node $i$ with $|R(i)| \in \{ 1, 2, 4\}$. We want to mention, for $\alpha \in [5/3, 2)$ and $|R(i)| \in \{1, 2, 4\}$, if $j \in R(i)$ and $k(j) = \{ 1 \} \cup [2 +\infty)$, then $\Delta(i) \geq 0$, so we will just assume all $k(j) \in (1, 2)$ for the case of $\Delta(i) < 0$. 






% % \begin{algorithm*}
% % \caption{Combine groups if the size is less than 4}
% % \label{Algorithm47}
% % \begin{algorithmic}[1]
% % \Function {Combine}{$g$}
% %         \If{$\exists \alpha = \{k_1\}, \alpha' = \{k_2, k_3, k_4 \} \in g(i)$ or $\exists \alpha = \{k_1, k_2\}, \alpha' = \{k_3, k_4 \} \in g(i)$}
% %             \State \Comment{combine group with size 1 and size 3 or group with size 2 and size 2}
% %             \State $\hat{\alpha} = \{k_1, k_2, k_3, k_4 \}$
% %             \If{$k_{j_1}, k_{j_2}$ are red}
% %                 \If{$rp(\hat{\alpha}) \le \frac{7k(\hat{\alpha})}{4}$}
% %                 \State $x_{k_{j_1}} \leftarrow \ceil{x_{k_{j_1}}}, x'_{k_{j_2}} \leftarrow \ceil{x'_{k_{j_2}}}$
% %                 \State $color(x'_{k_{j_1}}) \leftarrow black, color(x'_{k_{j_2}}) \leftarrow black$
% %                 \Else
% %                     \State $x'_{k_{j_1}} \leftarrow \ceil{x_{k_{j_1}}}, color(x'_{k_{j_1}}) \leftarrow black$
% %                 \EndIf
% %             \EndIf
% %             \If{only one $k_j$ is red,  where $j \in \{1, 2, 3, 4\}$}
% %                 \If{$rp(\hat{\alpha}) \le \frac{7k(\hat{\alpha})}{4}$}
% %                     \State $x'_{k_j} \leftarrow \ceil{x_{k_j}}, color(x'_{j}) \leftarrow black$
% %                 \EndIf
% %             \EndIf
% %             \If{$k_1, k_2, k_3, k_4$ are all black and $t'(\hat{\alpha}) - k(\hat{\alpha}) < 10/ 7$}
% %                     \State $x'_{k_1} \leftarrow x'_{k_1} + \ceil{10/ 7 - t'(\hat{\alpha}) + k(\hat{\alpha})}$
% %             \EndIf
% %         \EndIf
% %         \If{$\exists \alpha =  \{k_1\}, \alpha' = \{k_2, k_3 \} \in g(i)$}
% %             \Comment{combine group with size 1 and size 2}
% %             \State $\hat{\alpha} = \{k_1, k_2, k_3\}$
% %             \If{$k_1, k_j$ are red,  where $j \in \{2, 3\}$}
% %                 \If{$rp(\hat{\alpha}) \le \frac{7k(\hat{\alpha})}{4}$}
% %                 \State $x'_{k_1} \leftarrow \ceil{x_{k_1}}, x'_{k_j} \leftarrow \ceil{x_{k_j}}$
% %                 \State $color(x_{k_1}) \leftarrow black, color(x'_{k_j}) \leftarrow black$
% %                 \Else
% %                     \State $x'_{k_1} \leftarrow \ceil{x_{k_1}}, color(x'_{k_1}) \leftarrow black$
% %                 \EndIf
% %             \EndIf
% %             \If{only one $k_j$ is red,  where $j \in \{1, 2, 3\}$}
% %                 \If{$rp(\hat{\alpha}) \le \frac{4k(\hat{\alpha})}{7}$}
% %                     \State $x'_{k_j} \leftarrow \ceil{x_{k_j}}, color(x'_{j}) \leftarrow black$
% %                 \EndIf
% %             \EndIf
% %             \If{$k_1, k_2, k_3$ are all black and $t'(\hat{\alpha}) - k(\hat{\alpha}) < 4/ 7$}
% %                     \State $x'_{k_1} \leftarrow x'_{k_1} + \ceil{4/ 7 - t'(\hat{\alpha}) + k(\hat{\alpha})}$
% %             \EndIf
% %         \EndIf
% %         \If{$\exists \alpha = \{k_1\}, \alpha' =  \{ k_2 \} \in g(i)$}
% %             \Comment{combine group with size 1 and size 1}
% %             \State $\hat{\alpha} = \{k_1, k_2\}$
% %             \If{$k_1, k_2$ are both red}
% %                 \If{$rp(\hat{\alpha}) \le \frac{7k(\hat{\alpha})}{4}$}
% %                 \State $x'_{k_1} \leftarrow \ceil{x_{k_1}}, x'_{k_2} \leftarrow \ceil{x_{k_2}}$
% %                 \State $color(x'_{k_1}) \leftarrow black, color(x'_{k_2}) \leftarrow black$
% %                 \Else
% %                     \State Let $j \in [1, 2]$ be the node whose leaf node contains few jobs inside(If ties, choose a random node).
% %                     \State $x'_{k_j} \leftarrow \ceil{x_{k_j}}, color(x'_{k_j}) \leftarrow black$
% %                 \EndIf
% %             \EndIf
% %             \If{only one $k_j$ is red,  where $j \in \{1, 2\}$}
% %                 \State $x'_{k_j} \leftarrow \ceil{x_{k_j}}, color(x'_{j}) \leftarrow black$
% %             \EndIf
% %         \EndIf
% %         \If{we go to either of above 4 condition}
% %             \State $g \leftarrow g \cup \{ \hat{\alpha }\} / \{\alpha, \alpha'\}$
% %         \EndIf
% % \EndFunction
% % \end{algorithmic}
% % \end{algorithm*}

==> old-files/grouping.tex <==
\subsection{Grouping}
\label{subsection:grouping}

This section will describe an algorithm to partition the nodes of the tree into small subgroups.  This phase begins with the binary tree that is produced in Section \ref{subsection:linearprogram} from the linear program and the subsequent transformations on the tree.

The partitioning algorithm is shown in Algorithm \ref{alg:partition}.  The output is a partitioning of  the non-empty tree nodes.


The rounding starts from the root of the tree an recurses until it reaches the leaves.  At the end of the of the algorithm each non-empty node is assigned to a subgroup that contains at least 3 nodes, and at most 6 nodes, in total.






\begin{algorithm*}
\caption{Algorithm to partition the tree into groups\\
Input: The resulting binary tree from running the LP on an active time instance and a paramter $\tau$.\\
Output: A partitioning $P$ of the nodes into disjoint groups.}
\label{alg:partition}
\begin{algorithmic}[1]


\Function {Partition-Recurse}{$root, carry$}
    \If{$|root| \leq 2\tau$}
        \State $P \leftarrow P \cup \{carry \cup root \}$
    \ElsIf{$|root.left| \leq \tau$}
        \State $carry \leftarrow carry \cup root.left$
        \If{$|carry| \leq \tau$ }
            \State \Call{Partition-Recurse}{$root.right$, $carry$}
        \Else
            \State $P \leftarrow P \cup \{carry \}$
            \State \Call{Partition-Recurse}{$root.right$, \{\}}
        \EndIf
    \ElsIf{$|root.right| \leq \tau$}
        \State $carry \leftarrow carry \cup root.right$
        \If{$|carry| \leq \tau$ }
            \State \Call{Partition-Recurse}{$root.left$, $carry$}
        \Else
            \State $P \leftarrow P \cup \{carry\}$
            \State \Call{Partition-Recurse}{$root.left$, \{\}}
        \EndIf
    \Else
        \State \Call{Partition-Recurse}{$root.left$, $carry$}
        \State \Call{Partition-Recurse}{$root.right$,\{\} }
    \EndIf
    
\EndFunction
\end{algorithmic}
\end{algorithm*}

==> old-files/rounding.tex <==
\subsection{Rounding Algorithm}
\label{subsection:rounding}
%Let $I = (k_1, k_2, ..., k_{|I|})$ be a sequence of top-most non-empty nodes. 
We break nodes in $I$ into three types. A node $i \in I$ with $x(\Des(i)) = \theta$ (notice that $\theta \geq 1$) is of
		\begin{itemize}
			\item type-$\sfA$, if $\theta \geq 1.2$ and $\ceil{\theta} - \theta > 0.4$, 
			\item type-$\sfB$, if $\ceil{\theta} - \theta \leq 0.4$ (if $\theta = 1$, this condition is satisfied), 
			\item and type-$\sfC$, if $\theta \in (1, 1.2)$.
		\end{itemize}
		
		So, the interval $[1, \infty)$ is partitioned into 3 subsets as follows: $[1.2, 1.6) \cup (2, 2.6) \cup (3, 3.6) \cup (4, 4.6) \cup \cdots$ for type-$\sfA$ nodes,  $\{1\} \cup [1.6, 2] \cup [2.6, 3] \cup [3.6, 4] \cup \cdots$ for type-$\sfB$ nodes, and $(1, 1.2)$ for type-$\sfC$ nodes.
		
		We now explain the definitions. If $i$ is of type-$\sfA$ or type-$\sfB$, then we can afford to choose $\ceil{x(\Des(i))}$ slots in $\Des(i)$, since $\ceil{x(\Des(i))} / x(\Des(i)) \leq \frac53$.  For type-$\sfA$ node $i$, we gain at least 0.4 fractional extra slot by doing so.  For a type-$\sfB$ node $i$, we have $\frac53 x(\Des(i)) \geq \ceil{x(\Des(i))} + \frac23$. 
		
		So, the type-$\sfC$ nodes $i$ are those for which we can not freely round $x(\Des(i))$ up.  A type-$\sfC$ node $i$ is either a leaf in the tree, or a node with exactly child $i'$, which is a leaf satisfying $x(i') = L(i') = 1$.
		
		Now we shall define an integral vector $\tilde x$ which we obtain by rounding $x$. Instead of defining the integral vector $\tilde y$ explicitly, later we prove that $\tilde x$ satisfies all the necessary covering inequalities, which implies there is feasible integral solution $(\tilde x, \tilde y)$.
		
		For nodes $i \notin I$, we define $\tilde x(i) = x(i)$ since $x(i)$ is an integer. For a type-$\sfA$ or type-$\sfB$ node $i \in R$, we let $\tilde x(\Des(i)) = \ceil{x(\Des(i))}$, or equivalently, $\tilde x(i) = \ceil{x(i)}$.  It remains to define $\tilde x(i)$ for type-$\sfC$ nodes $i \in I$. 
		
		%Recall $I = (k_1, k_2, ..., k_{|I|})$ is the nodes in $I$ after ordering.
	
	\begin{itemize}[leftmargin=*]
		\item For every type-$\sfB$ node $i$, we choose the two type-$\sfC$ nodes $i'$ and $i''$ that are genetically closest to $i$, breaking ties by choosing the closest to $i$ in the sequence $I$. We force $\tilde x(\Des(i')) = \ceil{x(\Des(i'))} = 2$ and $\tilde x(\Des(i'')) = \ceil{x(\Des(i''))} = 2$.
		
		\item We then list all the type-$\sfC$ nodes in $I$ that are not forcibly rounded up from left to right, as $r_1, r_2, \cdots, r_o$. For every integer $p \in [0, o]$, let $z_p = \frac53\sum_{p' = 1}^p x(\Des(r_{p'}))$. For each $p \in [o]$, we define $\tilde x(r_p)$ so that $\tilde x(\Des(r_p))$ is the number of integers in the real interval $(z_{p-1}, z_p]$. As $z_p - z_{p-1} = \frac53x(\Des(r_p)) \in (\frac53, 2)$, we have $\tilde x(\Des(r_p)) \in \{1,2\}$. In other words, for every 0.6 fractional slot we see, we open 1 integral slot. 
	\end{itemize}
		
	Based on the value of $\tilde x(\Des(i))$, we further divide type-$\sfC$ nodes into type-$\sfC_1$ and $\sfC_2$ nodes.  $i$ is of type-$\sfC_1$ if $\tilde x(\Des(i)) = 1$ and of type-$\sfC_2$ if $\tilde x(\Des(i)) = 2$.  This finishes the description of $\tilde x$. The following lemma shows the rounding scheme is at most $\frac{5}{3}$ times the lp solution.
	
	\begin{lemma}
    After running the Algorithm described above, $\sum_{i} \tilde x(i) \leq \frac{5}{3} \sum_{i} x(i)$.
    \end{lemma}
    \begin{proof}
    We round up nodes in $I$, if $i \in I$ is a type-$\sfA$ node, rounding up $i$ doesn't violates the ratio. If $i$ is a type-$\sfB$ node, we will force at most two type-$\sfC$ node rounding up, notice that for $\sfC$ nodes $i, i''$, we have $x(i'), x(i'') \in (1, 1.2)$, so $\tilde x(i) + \tilde x( i' ) + \tilde x(i'') = \tilde x(i) + 4 \leq \frac53(x(i) + 2) \leq \frac53  (x(i) + \tilde x( i' ) + \tilde x(i''))$. For the remaining type-$\sfC$ nodes, we never violate the ratio. Each node lies on one of the three cases, so $\sum_{i} \tilde x(i) \leq \frac{5}{3} \sum_{i} x(i)$.
    \end{proof}


% After running the LP and applying the subsequent transformations on the tree from Section \ref{subsection:linearprogram}, we are left with a tree and solution that still has some fractional nodes.  In this section, we will show an algorithm which rounds the solution in order to get a set of open time slots which are all integers.  The algorithm has a parameter $\alpha$ which is the approximation ratio.
% The output is a set of open time slots $(X') = (x'_1, x'_2, ..., x'_m)$, which is a feasible solution to the problem.  The algorithm is shown in Algorithm \ref{alg:rounding}.




% The algorithm starts by recursing until it reaches a node in $R$.
% For each node $i \in R$, define the set of jobs assigned to a node according to the LP solution after the transformation as $t'(i) = \sum_{j\in Des(i)} x'(j)$. For $i \in R$, if $t(i) = 1$ or $t(i) \geq 2$, then round up the node, i.e. $x'(i) = \ceil{x(i)}$ and $\id{state}(i) = \id{up}$.  For the rest of the nodes $i \in R$, round the node $i$ down, i.e. $x'(i) = \floor{x(i)}$ and $\id{state}(i) = \id{down}$.  Rounding up a node opens up part of a time slot, and rounding down closes part of a time slot.  The nodes that are rounded up stay rounded up for the rest of the algorithm.  Next, the algorithm will choose some of the nodes that were rounded down to reopen in order to to fit the jobs that were scheduled by the LP in the slots that were closed.

% In the next part, the algorithm will process nodes that are not in $R$, once both of its children have been processed.
% To process a node $i \notin R$, round up a node in $R(i)$ whenever rounding up the a node doesn't violate the approximation ratio $\alpha$.  In particular, for $i \notin R$, if $t'(R(i))+1 \leq \alpha t(R(i))$, and there is a node in $R(i)$ that was rounded down, then a node in $R(i)$ is rounded up.
% For $|R(i)| > 2$, any node with state $\id{down}$ can be rounded up.  For $|R(i)| = 2$, the specific choice of which node to round up is important.  In particular, the node with the least jobs scheduled in it is rounded up.



% %The algorithm has a parameter $\alpha$ which is the approximation ratio.


% % The algorithm will starts with the nodes that are in $R$, and then move up the tree until reaching the root.  It will ignore nodes that are descendants of $R$.

% some nodes near the bottom of the tree, and process nodes moving up the tree.  It will round some nodes up, and some down so that by the end all the nodes have integral values.  At the end the algorithm outputs a new solution $(X', Y') = (x'_1, x'_2, ..., x'_m, y'_{1,1}, ..., y'_{m, n})$.


% Starting with the nodes in $R$, if $i \in R$, and, $t(i) = 1$ or $t(i) \geq 2$, then round up the time slot in the node, i.e. $x'_i = \ceil{x_i}$.  These nodes won't be changed for the rest of the algorithm.  Now, for the remaining nodes $i \in R$, (all are such that $1 < t(i) \leq 2$), round $i$ down i.e. $x'(i) = \floor{x(i)}$.  Next the algorithm will choose some of the nodes that it just closed to reopen.



 




% The algorithm starts at nodes in $R$. For the base case, i.e, the node $i \in R$, if $t(i) == 1$ or $t(i) \geq 2$, we will simply rounding up $x_i$ to $\ceil{x_i}$.Notice that once we finish the base case, now, only nodes with $1 < t(i) \leq 2$ left. Now we need to round some of those nodes up. When we process node $i \notin R$, we will always round up a node from $R(i)$ whenever rounding up a node doesn't violates the rounding ratio. Which node to round up is a problem for the algorithm. For now, assume we round up a random node. For the algorithm, we have a potential value $p$ for each node. We will set $p(i) = t'(i) - t(i)$ for $i \in R$ if we round it up. Notice that if we round a node up, then we have $p(i)$ time slot left. We still have the case that some nodes are rounded down, for those nodes, we will set $p(i) = -t(i)$. For an internal node $i$, we will set $p(i) = p(leftchild(i)) + p(rightchild(i)) = \sum_{j \in R(i)} p(j)$. Intuitively, when $p(i) < 0$, we need an extra $|p(i)|$ space to hold the jobs in $t(i)$. For $\alpha = 1.75$, we want to show after we process all nodes, $p(i) > 0$ for all nodes $i$ such that $|R(i)| > 2$. Thus, we only need to consider 2 special cases, when $|R(i)| == 1$ and $|R(i)| == 2$. For the first case, since we have the lp ceiling constraint, so we could always fit all jobs in $Des(i)$ into new time slot, we still need an extra $|p(i)|$ space to fit the jobs inn $Anc(i) / {i}$, but we could fit into any time slot. The second case, i.e, $|R(i)| == 2$ is a bit complicated. We will show that whenever $p(i) < 2$ and $|R(i)| == 2$, we could close the time slot such that the left node of that node contains more nodes and rounding up the other onne. We will show that all jobs with length less than or equal $2$ could be fitted into new time slot and thus we only need to assign jobs in $Anc(i) / {i}$ and the size the jobs need to be assigned is $|p(i)|$. 


% we will partition those nodes into different groups and each group contains at most 4 nodes. When we start from the base case, we mark all nodes in $R$ as red color. For each red node, if $t(i) \in \{1\} \cup [9/7, +\infty]$, we will round up the $x_i$ value and mark the color as black. The node from $R$, it only contains one descendant in $R$, itself, so we put itself into a group with size 1.


% Recall each node has at most two children nodes. If both children has been processed, we can process this node. When left child and right child both contain group with size 1, we will try to combine it and put those two nodes into group with size 2; when left child contains group with size 1 and left child contains group with size 2 or size 3, we will combine it to group with 3, or 4. When left child and right child both contain group with size 2, we will try to combine it and put those nodes into group with size 4; When we combine different group from children node, we will round up some of the red nodes and make sure it never violates the approximate ratio. Finally, there will be some nodes in $R$ still red, for those nodes, we will just round it down. 


% \begin{algorithm*}
% \caption{$\alpha$-approximate algorithm \\
% Input: The problem tree, an LP solution $(X, Y)$ and the nodes set $R$ \\
% Output: A set of time slots $X' = (x'(1), x'(2), ..., x'(m))$ where all $x'(i)$ are integers}
% \label{alg:rounding}
% \begin{algorithmic}[1]
% \Function {RoundingUp}{$Tree, (X, Y), R$}
%     \State \Call{RoundRecurse}{$tree.root$}
% \EndFunction 
% \vspace{-2ex}
% \Statex
% \Function{RoundRecurse}{node $i$}
%     \If{$i \in R$}
%         \If{$t(i) \in \{ 1 \} \cup [2, +\infty)$} $state(i) \leftarrow up, x'(i) \leftarrow \ceil{x(i)}$
%         \Else{} $state(i) \leftarrow down, x'(i) \leftarrow \floor{x(i)}$
%         \EndIf
%     \Else %i not in R, recurse
%         \State \Call{RoundRecurse}{$i.\id{left}$}
%         \State \Call{RoundRecurse}{$i.\id{right}$}
%         \While{$t'(i) + 1 \leq \alpha t(i)$ and at least one node in $R(i)$ has state $\id{down}$}
%             \State Let $j$ be an arbitrary node from $R(i)$ such that $state(j) = down$
%     \If{$|R(i)| == 2$ and both nodes have state down} 
%         \State $j = \argmin_{\{k | k \in R(i) \}}(|J(\id{Des}(k) \backslash \{ k \})|)$
%     \EndIf
%     % \If{$|R(i)| == 3$ and two nodes have state down} 
%     %     \State $j$ is the node in $R(i)$ such that $\not\exists k: j \in R(k) and |R(k)| = 2$
%     % \EndIf
%     \State $x'(j) \leftarrow \ceil{x(j)} , state(j) \leftarrow up$
%         \EndWhile
%     \EndIf
% \EndFunction
% \end{algorithmic}
% \end{algorithm*}


% \begin{algorithm*}
% \caption{$\alpha$-approximate algorithm \\
% Input: The problem tree, an LP solution $(X, Y)$ and the nodes set $R$ \\
% Output: A set of time slots $X' = (x'(1), x'(2), ..., x'(m))$ where all $x'(i)$ are integers}
% \label{alg:rounding3}
% \begin{algorithmic}[1]
% \Function {RoundingUp}{$Tree, (X, Y), R$}
%     \State \Call{RoundRecurse}{$tree.root$}
% \EndFunction 
% \vspace{-2ex}
% \Statex
% \Function{RoundRecurse}{node $i$}
%     \If{$i \in R$}
%         \If{$t(i) \in \{ 1 \} \cup [2, +\infty)$} $state(i) \leftarrow up, x'(i) \leftarrow \ceil{x(i)}$
%         \Else{} $state(i) \leftarrow down, x'(i) \leftarrow \floor{x(i)}$
%         \EndIf
%     \Else %i not in R, recurse
%         \State \Call{RoundRecurse}{$i.\id{left}$}
%         \State \Call{RoundRecurse}{$i.\id{right}$}
%         \While{$t'(R(i)) + 1 \leq \alpha \cdot t(R(i))$ and at least one node in $R(i)$ has state down}
%             \State \Call{RoundUpOneNode}{$i$}
%         \EndWhile
%     \EndIf
% \EndFunction
% \vspace{-2ex}
% \Statex
% \Function {RoundUpOneNode}{$i$}
%     \State Let $j$ be an arbitrary node from $R(i)$ such that $state(j) = down$
%     \If{$|R(i)| == 2$ and both nodes have state down} 
%         \State $j = argmin_{\{k | k \in R(i) \}}(|J(\id{Des}(k) \backslash \{ k \})|)$
%     \EndIf
%     \State $x'(j) \leftarrow \ceil{x(j)} , state(j) \leftarrow up$
% \EndFunction
% \end{algorithmic}
% \end{algorithm*}


% \begin{algorithm*}
% \caption{$\alpha$-approximate algorithm \\
% Input: The problem tree, an LP solution $(X, Y)$ and the nodes set $R$ \\
% Output: A set of time slots $X' = (x'(1), x'(2), ..., x'(m))$ where all $x'(i)$ are integers}
% \label{alg:rounding2}
% \begin{algorithmic}[1]
% \Function {RoundingUp}{$Tree, (X, Y), R$}
%     \State $P \leftarrow \{ \}$
%     \ForEach{$i \in R$}
%         \If{$t(i) \in \{ 1 \} \cup [2, +\infty]$}
%             \State $state(i) \leftarrow up, x'(i) \leftarrow \ceil{x(i)}$
%         \Else
%             \State $state(i) \leftarrow down, x'(i) \leftarrow \floor{x(i)}$
%         \EndIf
%         \State $P \leftarrow P \cup \{ i.parent \}$
%     \EndFor
%     \While{$P$ is not empty}
%         \State Choose node $i$ from $P$ such that $P \cap Des(i) = \emptyset$ %\Comment{process node from bottom to up}
        
%         \If{$i$ has two children}
%             \While{$t'(R(i)) + 1 \leq \alpha \cdot t(R(i))$ and $down \in state(R(i))$}
%                 \State RoundUpOneNode($i$)
%             \EndWhile
%         \EndIf
%         \State $P \leftarrow P \cup \{ i.parent \}$
%     \EndWhile
% \EndFunction
% \Function {RoundUpOneNode}{$i$}
%     \State Let $j$ be an arbitrary node from $R(i)$ such that $state(j) = down$
%     \If{$|R(i)| == 2$ and both nodes have state down} 
%         \State $j = argmin_{\{k | k \in R(i) \}}(|J(\id{Des}(k) \backslash \{ k \})|)$
%         % \Else
%         % \State Choose 
%         % \State $j = argmax_{\{k | k \in R(i), p(k) < 0\}}(|R(k)|)$.
%         % \While{$j \notin R(i)$}
%         %     \If{j contains only one child}
%         %         \State $j \leftarrow child(j)$
%         %     \ElsIf{only one child $c$ of $j$'s p value is negative}
%         %         \State $j \leftarrow c$
%         %     \Else
%         %         \State Let $c$ be the child contains more nodes in $R$
%         %         \State $j \leftarrow c$
%         %     \EndIf
%         % \EndWhile
%     \EndIf
%     \State $x'(j) \leftarrow \ceil{x(j)} , state(j) \leftarrow up$
%     % \State update $p$ value from node $k_j$ to i.
% \EndFunction
% \end{algorithmic}
% \end{algorithm*}

==> old-files/smallcases.tex <==
% Now that we've shown the case where $R(i)$ for node $i$ is large, we turn our attention to small $R(i)$.
% For $\alpha \in [7/4, 2)$, we already showed that for any $i \in D$, $|R(i)| \leq 2$.  Thus, we only need to consider the cases where $|R(i)| = 1$ and $|R(i)| = 2$. For the first case, since we have the LP ceiling constraint, we can always fit all jobs in $\id{Des}(i)$ into new time slot, we still need an extra $|\Delta(i)|$ space to fit the jobs in $\id{Anc}(i) \backslash \{i \}$. This gives us the following lemma, 

% %  For $\alpha = 1.75$,  we have that any $R(i) \geq 3$ has $\Delta(i) \geq 0$, so we only need to show that for $R(i) = 1$ or $R(i) = 2$, $i$ is $\Delta$-scheduled. The first case is $R(i)=1$ is shown in the following lemma.

% \begin{lemma}
% \label{onerednode}
% Consider a node $i \in D$ with $|R(i)| = 1$, $i$ is $\Delta$-scheduled.
% \end{lemma}

% The second case, i.e, $|R(i)| = 2$ is a bit complicated.  We will show that for any node $i$ such that $|R(i)| = 2$ and $t(i) < 5/2$, if we close the time slot $i_r$ such that the left node of that node contains more jobs in the descendant tree and rounding up the other one $i_l$, all jobs with length less than or equal $2$ can  fit into new time slot $t'(i_l)$ and $t'(i_r)$. This claim is given in the following lemma.
% \begin{lemma}
% \label{twonodes}
% Consider a node $i$ which contains exactly two time slots $i_l, i_r \in R(i)$ such that $t(i_l), t(i_r) \in (1, 2)$ and $t(i) = t(i_l)+ t(i_r) < 5/2$. Assume $|J(\id{Des}(i_l)) \backslash \{ i_l \}| \leq |J(\id{Des}(i_r) \backslash \{ i_r \}|$, i.e, $i_l$ contains fewer jobs in its descendant tree. Given a job assignment $Y(i)$, such that $l(Y(i), j)) \leq 2$ for all $j \in J$, i.e, the length of jobs assigned to time slot $i_l, i_r $ is at most 2. If we round up $i_l$ and round down $i_r$, for the new time slot $t'(i_l) = 2$ and $t'(i_r) = 1$, there exists a job assignment $Y'(i)$ for the new time slot such that $Y'(i) = Y(i)$.
% \end{lemma}

% We will leave Lemma \ref{twonodes} to prove later, but we will use it to prove the following lemma.

% \begin{lemma}
% \label{twonodeisscheduled}
% Consider a node $i \in D$ with $|R(i)| = 2$, for $\alpha \in [5/3, 2)$, $i$ is $\Delta$-scheduled.
% \end{lemma}
% \begin{proof}
% For a given node $i$ with $\Delta(i) < 0$ and $|R(i)| = 2$. let $i_l, i_r \in R(i)$ be nodes from $R$ in the subtree rooted at $i$. If $t(i_l), t(i_r) \in [1] \cup [2, +\infty)$, the algorithm will round up both nodes. Thus, we know that $t(i_l), t(i_r) \in (1, 2)$. On the other hand, since $\Delta(i) < 0$, we will round up exactly one of $i_l, i_r$. If we round up both $i_l, i_r$, the algorithm will violates the approximate ratio. Thus $\alpha \cdot t(i) < 4$ and $t(i) < 12 / 5$.

% As Algorithm \ref{alg:rounding} runs, consider the lowest node $k$ such that $R(i) = R(k)$ and $k \in \id{Des}(i)$.  The algorithm will round one node up and one node down. Assuming that there are fewer jobs in the $J(\id{Des}(i_l) \backslash \{ i_l \})$ than $J(\id{Des}(i_r) \backslash \{ i_r \})$, Algorithm \ref{alg:rounding} always rounds up the time slot $t(i_l)$ to $t'(i_l) = 2$. The node $i_r$ will be rounded down to $t'(i_r) = 1$.

% Now for the job assignment $Y(i)$, the length of jobs in $\id{Des}(i)$ is at most 2. Otherwise, the first constraint in the LP will force $t(i)$ to be 3. 
% For a job $j \in \id{Anc}(i) \backslash \{ i \}$, the length assigned to the time slot $l(Y(i), j)$ could be more than 2. 
% If $l(Y(i), j) > 2$, then we will only leave $2$ time slots of jobs in $Y(i)$ and remove $l(Y(i), j) - 2$ out of $Y(i)$. Notice that we only need an extra $t(i) - 2$ time slot to hold the jobs removed in this process.  
% Let $\bar{Y}(i)$ be the job assignment after removing jobs longer than 2. 
% By Lemma \ref{twonodes}, we know there exists a job assignment $Y'(i)$ for the new time slot such that $Y'(i) = \bar{Y}(i)$. 
% The new time slot is exactly the time slot our algorithm produces. 
% For the job assignment $Y'(i)$, all jobs in $\id{Des}(i)$ have been assigned and we only need an extra $t(i) - 2 = |\Delta(i)|$ extra time slots to hold jobs from $\id{Anc}(i) \backslash \{ i \}$. This is the definition of $\Delta$-scheduled.
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{1.75main}.]
% For $\alpha = 1.75$, Corollary \ref{175rsize} shows for any node $i$ such that $\Delta(i) < 0$ only if $|R(i)| < 3$. For the root node, if the $\Delta(root) < 0$, Lemmas \ref{onerednode} and \ref{twonodeisscheduled} tell us all jobs in $\id{Des}(root)$ can be scheduled. Otherwise, we can use Lemma \ref{allnodesscheduled} to we could schedule all jobs in the set of time slots. Either way, the schedule is feasible.
% \end{proof}

% \paragraph*{Main idea of the proof of Lemma \ref{twonodes}.}
% The full proof of Lemma \ref{twonodes} is in the Appendix.  The proof gets long and complicated but we will describe main idea here.  There are two times slots for $i$, $i_l$ and $i_r$, that we are trying to schedule jobs into.
% Since $t(i_l), t(i_r) \in (1, 2)$, both of $i_l$ and $i_r$ contain one leaf node with one unit time slot.
% For the nodes from $\id{Des}(i_l) \backslash \{ i_l \}$ and $\id{Des}(i_r) \backslash \{ i_r \}$ the jobs inside must use the leaf time slots. 
% Let $k$ be the lowest node that contains $i_l$ and $i_r$. The nodes in $\id{Des}(k) \cap \id{Anc(i_l)} \backslash \{ k \} $, $\id{Des}(k) \cap \id{Anc(i_r)} \backslash \{ k \} $ have more flexibility in where they can be scheduled.  
% The length of the jobs inside is also 1 due to the ceiling constraint of the LP, but they have more choice in which node to be assigned to. 
% The jobs in $\id{Des}(k) \cap \id{Anc(i_l)} \backslash \{ k \}$ can be put into $x(i_l)$ or the leaf node time slot. 
% Lastly, for jobs in $\id{Anc}(k) \cap \id{Des(i)}$, they can be put into any time slot in the $R(i)$. The proof will argue that given a time slot, scheduling the jobs into the least used time slot always gives the "best" assignment of the jobs.  The idea of the "best" assignment is the assignment that allows for scheduling the jobs from higher in the tree.  To compare the job assignments, we define a time configuration and argue a better time configuration can schedule at least the jobs of the original time configuration. 
% Lastly, we schedule the jobs $\id{Des}(k) \backslash \{ k \}$ into $t(i_l), t(i_r)$ and $t'(i_l), t'(i_r)$ using a greedy strategy.






% % \begin{lemma}
% % After we process node $i$, assume the group for $i$ is $g(i) = \{ \alpha_1, \alpha_2, ..., \alpha_l \}$, where $|\alpha_1| \leq |\alpha_2| \leq ... \leq |\alpha_l|$ and $l \geq 2$. For each $\alpha_j$, $j \in [2, l]$, there will be at most 1 red node. Besides, one of the following happens:
% % \begin{itemize}
% %     \item $|\alpha_1| == 1$ and $|\alpha_j| == 4$ for all $j\in [2,l]$
% %     \item $|\alpha_1| \geq 2$ and $|\alpha_j| \geq 3$ for all $j\in [2,l]$
% % \end{itemize}
% % \end{lemma}

% % \begin{proof}
% % Omitted.
% % \end{proof}




% % \begin{corollary}
% % \label{tworednode}
% % Consider a Node $i$ with containing one red node and one black node. Then we could put  $j \in J(Des(i))$ into $t'(i)$. Besides, there might be some jobs $j \in J(Anc(i) / \{ i \})$ putting into time slot $t(i)$, for those part value, we need an extra $t(i) - 2$ slot to hold it.
% % \end{corollary}

% % Notice that for those two cases, we allow an extra slot to hold it. That's because we could already hold all jobs $J(Des(i))$ into the new time slot. We still need some time slot to hold the remaining jobs, but if we can find some unused slot when the node contains 3 or more nodes in $R$, then it's still a feasible solution. We use $\mu(i)$ to represent the time slot needed or unused, if $\mu(i) < 0$, it means we need $|\mu(i)|$ time slot. Otherwise, we have unused $\mu(i)$ time slot. For the base case, all black node is set to be $\mu(i) = t'(i) - t(i) \geq 0$. All red node is set to be $\mu(i) = - t(i) < 0$. This comes from the lemma \ref{onerednode}. Now if a node contains only one child node, we just use its child $\mu$ value as itself $\mu$ value. In the case of a node contains two child node, we will update the $x'$ value and the corresponding $\mu$ value for the whole path. Now the node's $\mu(i) = \mu(left(i)) + \mu(right(i))$. Notice that if the node only contains black node, then $\mu$ is valid. Otherwise, the node contains one black node and one red node. In this case, corollary \ref{corollary} told us we need an extra $t(i) - 2$ time slot, and $\mu$ should be set to $\mu = 2 - t(i)$. $\mu(i) = \mu(left(i)) + \mu(right(i))$ makes the $\mu = 2 - t(i)$. Now when the algorithm processes a node, if it contains only one child, we will use its child $\mu$ value, otherwise, set $\mu(i) = \mu(left(i)) + \mu(right(i))$. For all nodes containing more than $2$ $R$'s node, if it's $\mu < 0$, then algorithm fails. Otherwise, there will be $\mu(i)$ unused time slot. This makes the following lemma:


% % Consider group with size $1$, i.e, $\alpha = (k_1) \in g$. We will only round it up when $t(k_1) \in \{1\} \cup [9/7, +\infty]$. In this case
% % \begin{equation*}
% %     t'(k_1) = t(k_1) - x_{k_1} + \ceil{x_{k_1}} \leq \frac{7}{4} t(k_1)
% % \end{equation*}
% % If $t(k_1) \in (1, 9/7)$, we will round down $x_{k_1}$, thus $t'(k_1) \leq t(k_1)$.

% % Next, we will have group with size $2$ if we have 2 group with size 1. Let $\alpha = (k_1, k_2) \in g$ be such group, We will round up $k_1$ or $k_2$ only if one of $k_1$ and $k_2$ are red node. If only one node is red, let $k_1$ be such node, we have $t(k_1) \in (1, 9/7), t(k_2) \in \{1\} \cup [9/7, +\infty]$. If $t(k_2) ==  1$, then rounding up $k_1$ will never violate our approximate ratio. Otherwise, $t(k_2) \geq 9/7$ and $t(\alpha) \geq 16 / 7$.
% % \begin{equation*}
% %     t'(\alpha) = t(\alpha) + \ceil{x_{k_1}} + \ceil{x_{k_2}} - x_{k_2} - x_{k_1} +  \leq \frac{7}{4} t(\alpha)
% % \end{equation*}
% % Last, if both $k_1$ and $k_2$ are red node, if rounding up both doesn't violate the ratio, we will round them up. Otherwise, we only round up one of then, notice that $t(k_1), t(k_2) \in (1, 9/7)$, rounding up one of them never violate the ratio.

% % For the group with size 3. Let $\alpha = (k_1, k_2, k_3) \in g$ be such group
% % \begin{itemize}
% %     \item after processing this group, all nodes become black, in this case, $t'(\alpha) \leq \frac{7}{4}t(\alpha)$. If $t'(\alpha) - t(\alpha) < 4 /7$. This never violate the approximate ratio
% %     \item two red nodes become 1 red node. this case doesn't violate the ratio.
% %     \item $k_1$ is red node and it keeps red. this case doesn't violate the ratio.
% % \end{itemize}

% % For the group with size 4. Let $\alpha = (k_1, k_2, k_3, k_4) \in g$ be such group
% % \begin{itemize}
% %     \item after processing this group, all nodes become black, in this case, $t'(\alpha) \leq \frac{7}{4}t(\alpha)$. If $t'(\alpha) - t(\alpha) < 10 /7$. This never violate the approximate ratio.
% %     \item 1 red node Left. this case doesn't violate the ratio.
% % \end{itemize}
% % Combining all cases, when all groups will violate our ratio and finally, each node in $R$ will be in some group, so the ratio never violates 1.75 ratio.
% % \end{proof}

% % For each node $i$, let $\mu(i)$ be the extra time slot or unused slots if we use the new $X'$ instead of the $X$ time slot and we use the old $Y$. For example, for node $i \in R$, if we round up $x_i$ to $\ceil{x_i}$, then $\mu(i) = \ceil{x_i} - x_i$. On the other side, if we round down $x_i$ to $\ceil{x_i}$, we might need an extra $t(i)$ to hold the jobs previously in the slot $t(i)$. Notice, $t(i)$ could be much larger than $x_i$. The good news is that if for this $i$, if we round down it, it must be the case $t(i) \in (1, 9/7)$. After rounding, $t'(i) = 1$. We know that the job set $J(Des(i))$ contains at most $g$ jobs with length 1, if not, the integer constraint of the lp will force $t(i) \geq 2$. Having the constraint on $J(Des(i))$, we know, we could put all $y_{ij}$ for $j \in J(Des(i))$ into $t'(i)$. We still need an extra $t(x_i)$ time slot, but if we can find this amount of time slot on the rounding up slot, it will be fine to hold all $Y$. For the cases an node contains exact 2 nodes in $R$, we might still need some extra spaces. However, we prove that all jobs in the subtree could be satisfied and very little amount extra time slot is needed for jobs above this node. Then for other node, we will show there will be some unused slots. It's the same as proving $\mu(i) > 0$ for all other cases. To prove $\mu(i)$ value, we will prove that each group with size 3's $\mu \geq 4 /7$ and each group with size 4's $\mu \geq 10 / 7$. Notice that we already proved for each node, the possibilities of the group, combining this two thing together, we show $\mu(i) > 0$ for all nodes contains more than 3 $R$'s nodes, which implies the case a node contains 3  $R$'s node always has some unused space and all jobs could be arranged. 



% % The cases a node contains two $R$'s node is more complicated and it's our main lemma of the proof.


% % Now the only thing we want to prove is that $\mu > 0$ for all nodes containing more than 2 R's nodes.

% % \begin{lemma}
% % Considering the $\mu$ above, for any node $i$ contains at least 2 R's node, we have $\mu(i) > 0$.
% % \end{lemma}
% % \begin{proof}
% % The tricky part of the proof is that notice that when we count $\mu$ value for each node, for the base case, we just set $\mu(i) = t'(i) - t(i) \geq 0$ for black node and set $\mu(i) = - t(i) < 0$ for red node. Later, each $\mu$ value is the summation of the children's $\mu$ value. Thus, 

% % \begin{equation*}
% %     \mu(i) = \sum_{j \in R \cap Des(i) }\mu(j) 
% % \end{equation*}
% % Notice that groups $g = \{ \alpha_1, \alpha_2, ..., \alpha_l\}$ is a partition of $Des(i)$, we will count $\mu(\alpha_j)$ for each $j \in [1, l]$.
% % \begin{itemize}
% %     \item For $\alpha_j = (k_1)$, we want to show $\mu(\alpha_j) \geq -9/7$.
% %     \item For $\alpha_j = (k_1, k_2)$, we want to show $\mu(\alpha_j) \geq -2/7$. Assume $k_1$ is red and $k_2$ is black, we have $t(k_1) + t(k_2) < 16 /7$ and $t(k_1)>1, t(k_2) > 1$, $\mu(\alpha_j) = 2 - t(k_1) - t(k_2) \geq -2/7$
% %     \item For $\alpha_j = (k_1, k_2, k_3)$, we want to show $\mu(\alpha_j) \geq 4/7$. $k_1$ is red, then we have $t(k_1) + t(k_2) + t(k_3) < 24 /7$ and $t(k_1)>1, t(k_2) > 1, t(k_3) > 1$ , $\mu(\alpha_j) = 2 + 2 - t(k_1) - t(k_2) - t(k_3) \geq 4/7$
% %     \item For $\alpha_j = (k_1, k_2, k_3, k4)$, we want to show $\mu(\alpha_j) \geq 10/7$.
% % \end{itemize}

% % \end{proof}

